Batch Policy Gradient Methods for Improving Neural Conversation Models

We study reinforcement learning of chatbots with recurrent neural network architectures when the rewards are noisy and expensive to obtain. For instance, a chatbot used in automated customer service support can be scored by quality assurance agents, but this process can be expensive, time consuming and noisy. Previous reinforcement learning work for natural language processing uses on-policy updates and/or is designed for on-line learning settings. We demonstrate empirically that such strategies are not appropriate for this setting and develop an off-policy batch policy gradient method (BPG). We demonstrate the efficacy of our method via a series of synthetic experiments and an Amazon Mechanical Turk experiment on a restaurant recommendations dataset.

==> DAP/dap_exp.tex <==

\section{Experiments}
\label{sec:experiments}

\textbf{Implementation Details:}
We implement our methods using Chainer~\citep{tokui2015chainer},
and group sentences of the same length together in the same batch to make use of GPU
parallelisation.
Since different batches could be of different length, we do not normalise the gradients
by the batch size as we should take larger steps after seeing more data. 
However, we normalise
by the length of the output sequence to allocate equal weight to all sentences.
We truncate all output sequences to length $64$ and use a maximum batch size of $32$.
We found it necessary to use a very small step size ($10^{-5}$), otherwise the
algorithm has a tendency to get stuck at bad parameter values.
% 
While importance re-weighting is necessary in off-policy settings, it can
increase the variance of the updates, especially when $q(\at|\st)$ is very small.
A common technique to alleviate this problem is to clip  the $\rho(\st,\at)$
value~\citep{swaminathan2015counterfactual}.
In addition to single $\rho(\st,\at)$ values, our procedure has a product
of $\rho(\st,\at)$ values when computing the future rewards~\eqref{eqn:rlambdat}.
The effect of large $\rho$ values is a large weight $\rhot(\rlambdat - \valfunhat(\st))$
for the score function in step (ii) of Algorithm~\ref{alg:logpolgrad}.
In our implementation, we clip this weight at $5$ which controls the variance of the
updates and ensures that a single example does not disproportionately affect the gradient.

\textbf{RNN Design:}
In both experiments we use deep LSTMs with two layers for the encoder and decoder
RNNs. 
The output of the bottom layer is fed to the top layer and in the decoder RNN,
the output of the top layer is fed to a softmax layer of size $|\Acal|$.
When we implement \gtdls to estimate $\valfunpt$ 
we use the hidden state of the bottom LSTM as $\phi(s)$.
When performing our policy updates, we only change  the parameters of the top LSTM
and the softmax layer in our decoder RNN. If we were to change the bottom LSTM too, then
the state representation $\phi(s)$ would also change as the policy changes.
This violates the MDP framework.
In other words, we treat the bottom layer as part of the environment in our MDP.
To facilitate a fair comparison, we only
modify the top LSTM and softmax layers in all methods.
We have illustrated this set up in Fig.~\ref{fig:lstmIllus}.
We note that if one is content with using the constant estimator,
then one can change all parameters of the RNN.

\insertFigLSTM


\subsection{Some Synthetic Experiments on the Europarl dataset}
\label{sec:expsyn}

To convey the main intuitions of our method, we compare our methods against other baselines
on a synthetic task on the European parliament proceedings
corpus~\citep{koehn2005europarl}.
We describe the experimental set up briefly, deferring details to
Appendix~\ref{app:syndetails}.
The input sequence to the RNN was each sentence in the dataset.
Given an input, the goal was to reproduce the words in the input without
repeating words in a list of forbidden words.
The RL algorithm does not explicitly know either goal
of the objective but has to infer it from the \emph{stochastic} rewards assigned 
to input output sequences in the dataset.
We used a training set of $500$ input-output-reward triplets for
the RL methods.

We initialised all methods by maximum likelihood training on
$6000$ input output
sequences where the output sequence was the reverse of the input sequence.
The maximum likelihood objective captures part of the RL objective.
This set up reflects naturally occurring practical scenarios for the algorithm where
a large amount unlabelled data can be used to bootstrap a policy
if the maximum likelihood and reinforcement learning objectives are at least partially
aligned. 
We trained the RL algorithms for $200$ epochs on the training set.
At the end of each epoch, we generated outputs from the policy on test set
of $500$ inputs
and scored them according to our criterion. We plot the test set error against
the number of epochs for various methods in Fig.~\ref{fig:synresults}.


Fig.~\ref{fig:ml} compares $3$ methods: \bpgs with and without maximum likelihood
initialisation and 
a version of \bpgs which does not use importance sampling.
Clearly, bootstrapping an RL algorithm with ML can be advantageous especially
if data is abundantly available for ML training.
Further, without importance sampling, the algorithm is not as competitive
for reasons described in Section~\ref{sec:comparison}.
In all $3$ cases, we used a constant estimator for $\valfunhat$ and $\lambda=0.5$.
The dashed line indicates the performance of ML training alone.
\bpgniss is similar to the algorithms of~\citet{williams2016end,ranzato2015sequence}
except that there, their methods implicitly use $\lambda=1$.

Fig.~\ref{fig:constvsgtdl} compares $4$ methods: \bpgs and its on-line version \opgs
 with constant (\const) and \gtdls estimators for $\valfunhat$.
The on-line  versions of the algorithms are a direct implementation of the method
in~\citet{degris2012offpac} which do not use the future rewards as we do.
The first observation is that while \gtdls is slightly better in the early iterations,
it performs roughly the same as using a constant estimator in the long run.
Second, \bpgs performs significantly better than \opg.
This should not be surprising --
a close inspection of~\citet{degris2012offpac} reveals that the algorithm sees the
reward only at the end of the episode. This is typical of many RL algorithms
where the reward appears in the update only at the time step it is realised.
For the reward to get factored into policy updates in earlier time steps, it has to
percolate through updates for the estimate of the value function $\valfunhat$.
While this is reasonable in on-line settings where we can explore indefinitely to collect 
a large number of samples and estimate $\valfunhat$,
it is difficult when one only has a limited number of labelled samples.
Finally, we compare \bpgs with different choices for $\lambda$ in Fig.~\ref{fig:difflambda}.
As noted previously, $\lambda<1$ is useful
with stochastic rewards, but choosing too small a value is detrimental.
The optimal $\lambda$ value may depend on the problem.

\insertFigSynOne




\subsection{Restaurant Recommendations}
\label{sec:exprestaurant}

We use data from an on-line restaurant recommendation service. Customers log into
the service and chat with a human agent asking recommendations for restaurants.
The agents ask a series of questions such as food preferences, group size
etc. before recommending a restaurant.
This dataset was obtained from Microsoft.
The goal is to train a chat-bot (policy) which can replace or assist the agent.
For reasons explained in Section~\ref{sec:intro}, maximum likelihood training alone will
not be adequate.
By obtaining reward labels for responses produced by various other bots,
we hope to improve on a bot initialised using maximum likelihood.


\textbf{Data Collection:}
We collected data for RL as follows.
We trained five different  RNN chat-bots with different LSTM
parameters via maximum likelihood  on a dataset of $6000$ conversations from this dataset.
The bots were trained to reproduce what the human agent said (output $y$) given the
past conversation history (input $x$).
Then, we generated responses from these bots on $1216$ separate conversations and had
them scored by workers on Amazon Mechanical Turk (AMT).
For each response by the bots in each conversation,
the workers were shown the history before the particular response and asked to
score (label) each response on a scale of $0-1-2$.
% $\bf 2$: the response is coherent and appropriate given the history;
% $\bf 1$: the response has some minor flaws but is discernible and appropriate;
% $\bf 0$: the response is completely incoherent or inappropriate.
We collected scores from three different workers for each response and used the mean as
the reward in our RL framework.


\textbf{Policies and RL Application:}
Next, we initialised $2$ bots via maximum likelihood and then used \bpgs to
improve them using the labels collected from AMT.
For the $2$ bots we used the following LSTM hidden state size $H$, word embedding size $E$
and \bpgs parameters.
These parameters were chosen arbitrarily and are different from those of the bots 
used in data collection described above.
% described in the  previous paragraph used for data collection.
% The details on the $2$ bots, which are different to the $5$ bots used for collecting
% the data, are as follows.
\begin{itemize}
\item {Bot-1}: $H=512$, $E=256$. $\quad$
\bpg: $\lambda = 0.5$,$\;$ \gtdls estimator for $\valfunhat$.
\item {Bot-2}: $H=400$, $E=400$. $\quad$
\bpg: $\lambda = 0.5$,$\;$ constant estimator for $\valfunhat$.
\end{itemize}

\textbf{Testing:}
We used a separate test set of $500$ conversations which had a total of more than
$3500$ input-output (conversation history - response) pairs.
For each Bot-1 and Bot-2 we generated responses before and after applying \bpg, totalling
$4$ responses per input.
% We generated $4$ responses on a separate dataset of $500$ conversations.
% The responses were from Bot-1 and Bot-2 before and after applying \bpg.
We then had them scored by workers on AMT using the same set up described above.
The same worker labels the before-\bpgs and after-\bpgs responses from the same bot.
This controls spurious noise effects and allows us to conduct a paired test.
We collected $16,808$ before and after label pairs each for Bot-1 and Bot-2 and
compare them using a paired t-test and a Wilcoxon signed rank test.

\textbf{Results:}
The results are shown in Table~\ref{tb:mturk}.
The improvements on Bot-2 are statistically significant at the $10\%$ level on both tests,
while Bot-1 is significant on the Wilcoxon test.
The large p-values for Bot-1 are due to the noisy nature of AMT experiments and we
believe that we can attain significance if we collect more labels
which will reduce the standard error in both tests.
Nonetheless, it appears that the improvements are small as evidenced by the mean
values. Exploring methods to improve these results further will be a pursuit 
for future work.
In Appendix~\ref{app:restaurantdetails} we present some examples of responses generated by
the bots before and after applying \bpg. 
We qualitatively discuss specific kinds of issues that we were able to overcome via
reinforcement learning.


\insertRealResultsNew


==> DAP/figsTables.tex <==




==> experiments.tex <==

\section{Experiments}
\label{sec:experiments}

\textbf{Implementation Details:}
We implement our methods using Chainer~\citep{tokui2015chainer},
and group sentences of the same length together in the same batch to make use of GPU
parallelisation.
Since different batches could be of different length, we do not normalise the gradients
by the batch size as we should take larger steps after seeing more data. 
However, we normalise
by the length of the output sequence to allocate equal weight to all sentences.
We truncate all output sequences to length $64$ and use a maximum batch size of $32$.
We found it necessary to use a very small step size ($10^{-5}$), otherwise the
algorithm has a tendency to get stuck at bad parameter values.
% 
While importance re-weighting is necessary in off-policy settings, it can
increase the variance of the updates, especially when $q(\at|\st)$ is very small.
A common technique to alleviate this problem is to clip  the $\rho(\st,\at)$
value~\citep{swaminathan2015counterfactual}.
In addition to single $\rho(\st,\at)$ values, our procedure has a product
of $\rho(\st,\at)$ values when computing the future rewards~\eqref{eqn:rlambdat}.
The effect of large $\rho$ values is a large weight $\rhot(\rlambdat - \valfunhat(\st))$
for the score function in step (ii) of Algorithm~\ref{alg:logpolgrad}.
In our implementation, we clip this weight at $5$ which controls the variance of the
updates and ensures that a single example does not disproportionately affect the gradient.

\textbf{RNN Design:}
In both experiments we use deep LSTMs with two layers for the encoder and decoder
RNNs. 
The output of the bottom layer is fed to the top layer and in the decoder RNN,
the output of the top layer is fed to a softmax layer of size $|\Acal|$.
When we implement \gtdls to estimate $\valfunpt$ 
we use the hidden state of the bottom LSTM as $\phi(s)$.
When performing our policy updates, we only change  the parameters of the top LSTM
and the softmax layer in our decoder RNN. If we were to change the bottom LSTM too, then
the state representation $\phi(s)$ would also change as the policy changes.
This violates the MDP framework.
In other words, we treat the bottom layer as part of the environment in our MDP.
To facilitate a fair comparison, we only
modify the top LSTM and softmax layers in all methods.
We have illustrated this set up in Fig.~\ref{fig:lstmIllus}.
We note that if one is content with using the constant estimator,
then one can change all parameters of the RNN.

\insertFigLSTM


\subsection{Some Synthetic Experiments on the Europarl dataset}
\label{sec:expsyn}

To convey the main intuitions of our method, we compare our methods against other baselines
on a synthetic task on the European parliament proceedings
corpus~\citep{koehn2005europarl}.
We describe the experimental set up briefly, deferring details to
Appendix~\ref{app:syndetails}.
The input sequence to the RNN was each sentence in the dataset.
Given an input, the goal was to reproduce the words in the input without
repeating words in a list of forbidden words.
The RL algorithm does not explicitly know either goal
of the objective but has to infer it from the \emph{stochastic} rewards assigned 
to input output sequences in the dataset.
We used a training set of $500$ input-output-reward triplets for
the RL methods.

We initialised all methods by maximum likelihood training on
$6000$ input output
sequences where the output sequence was the reverse of the input sequence.
The maximum likelihood objective captures part of the RL objective.
This set up reflects naturally occurring practical scenarios for the algorithm where
a large amount unlabelled data can be used to bootstrap a policy
if the maximum likelihood and reinforcement learning objectives are at least partially
aligned. 
We trained the RL algorithms for $200$ epochs on the training set.
At the end of each epoch, we generated outputs from the policy on test set
of $500$ inputs
and scored them according to our criterion. We plot the test set error against
the number of epochs for various methods in Fig.~\ref{fig:synresults}.


Fig.~\ref{fig:ml} compares $3$ methods: \bpgs with and without maximum likelihood
initialisation and 
a version of \bpgs which does not use importance sampling.
Clearly, bootstrapping an RL algorithm with ML can be advantageous especially
if data is abundantly available for ML training.
Further, without importance sampling, the algorithm is not as competitive
for reasons described in Section~\ref{sec:comparison}.
In all $3$ cases, we used a constant estimator for $\valfunhat$ and $\lambda=0.5$.
The dashed line indicates the performance of ML training alone.
\bpgniss is similar to the algorithms of~\citet{williams2016end,ranzato2015sequence}
except that there, their methods implicitly use $\lambda=1$.

Fig.~\ref{fig:constvsgtdl} compares $4$ methods: \bpgs and its on-line version \opgs
 with constant (\const) and \gtdls estimators for $\valfunhat$.
The on-line  versions of the algorithms are a direct implementation of the method
in~\citet{degris2012offpac} which do not use the future rewards as we do.
The first observation is that while \gtdls is slightly better in the early iterations,
it performs roughly the same as using a constant estimator in the long run.
Next, \bpgs performs significantly better than \opg.
% This should not be surprising --
% a close inspection of~\citet{degris2012offpac} reveals that the algorithm sees the
% reward only at the end of the episode. This is typical of many RL algorithms
% where the reward appears in the update only at the time step it is realised.
% For the reward to get factored into policy updates in earlier time steps, it has to
% percolate through updates for the estimate of the value function $\valfunhat$.
% While this is reasonable in on-line settings where we can explore indefinitely to collect 
% a large number of samples and estimate $\valfunhat$,
% it is difficult when one only has a limited number of labelled samples.
\modifone{
We believe this is due to the following two reasons.
First, the online updates assume stationarity of the MDP.
When this does not hold, such as in limited data instances like ours,
the SGD updates can be very noisy.
Secondly, the value function estimate plays a critical role in the online version.
While obtaining a reliable estimate $\valfunhat$ is reasonable in on-line settings where
we can explore indefinitely to collect a large number of samples,
it is difficult when one only has a limited number of labelled samples.
}
Finally, we compare \bpgs with different choices for $\lambda$ in Fig.~\ref{fig:difflambda}.
As noted previously, $\lambda<1$ is useful
with stochastic rewards, but choosing too small a value is detrimental.
The optimal $\lambda$ value may depend on the problem.

\insertFigSynOne




\subsection{Restaurant Recommendations}
\label{sec:exprestaurant}

We use data from an on-line restaurant recommendation service. Customers log into
the service and chat with a human agent asking recommendations for restaurants.
The agents ask a series of questions such as food preferences, group size
etc. before recommending a restaurant.
The goal is to train a chatbot (policy) which can replace or assist the agent.
For reasons explained in Section~\ref{sec:intro}, maximum likelihood training alone will
not be adequate.
By obtaining reward labels for responses produced by various other bots,
we hope to improve on a bot initialised using maximum likelihood.


\textbf{Data Collection:}
We collected data for RL as follows.
We trained five different  RNN chatbots with different LSTM
parameters via maximum likelihood  on a dataset of $6000$ conversations from this dataset.
The bots were trained to reproduce what the human agent said (output $y$) given the
past conversation history (input $x$).
\modifone{
While the dataset is relatively small, we can still expect our bots to do
reasonably well since we work in a restricted domain.
}
Next, we generated responses from these bots on $1216$ separate conversations and had
them scored by workers on Amazon Mechanical Turk (AMT).
For each response by the bots in each conversation,
the workers were shown the history before the particular response and asked to
score (label) each response on a scale of $0-1-2$.
% $\bf 2$: the response is coherent and appropriate given the history;
% $\bf 1$: the response has some minor flaws but is discernible and appropriate;
% $\bf 0$: the response is completely incoherent or inappropriate.
We collected scores from three different workers for each response and used the mean as
the reward.


\textbf{Policies and RL Application:}
Next, we initialised $2$ bots via maximum likelihood and then used \bpgs to
improve them using the labels collected from AMT.
For the $2$ bots we used the following LSTM hidden state size $H$, word embedding size $E$
and \bpgs parameters.
These parameters were chosen arbitrarily and are different from those of the bots 
used in data collection described above.
% described in the  previous paragraph used for data collection.
% The details on the $2$ bots, which are different to the $5$ bots used for collecting
% the data, are as follows.
\begin{itemize}
\item {Bot-1}: $H=512$, $E=256$. $\quad$
\bpg: $\lambda = 0.5$,$\;$ \gtdls estimator for $\valfunhat$.
\item {Bot-2}: $H=400$, $E=400$. $\quad$
\bpg: $\lambda = 0.5$,$\;$ constant estimator for $\valfunhat$.
\end{itemize}

\textbf{Testing:}
We used a separate test set of $500$ conversations which had a total of more than
$3500$ input-output (conversation history - response) pairs.
For each Bot-1 and Bot-2 we generated responses before and after applying \bpg, totalling
$4$ responses per input.
% We generated $4$ responses on a separate dataset of $500$ conversations.
% The responses were from Bot-1 and Bot-2 before and after applying \bpg.
We then had them scored by workers on AMT using the same set up described above.
The same worker labels the before-\bpgs and after-\bpgs responses from the same bot.
This controls spurious noise effects and allows us to conduct a paired test.
We collected about $7500$ before and after label pairs each for Bot-1 and Bot-2 and
compare them using a paired t-test and a Wilcoxon signed rank test.

\textbf{Results:}
The results are shown in Table~\ref{tb:mturk}.
The improvements on Bot-2 are statistically significant at the $10\%$ level on both tests.
\modifone{While the improvement on Bot-1 is not significant
we still see that it does better than the \mls bot}.
The large p-values for Bot-1 are due to the noisy nature of AMT experiments and we
believe that we can attain significance if we collect more labels
which will reduce the standard error in both tests.
In Appendix~\ref{app:restaurantdetails} we present some examples of conversation
histories and the responses generated by the
bots before and after applying \bpg. 
We qualitatively discuss specific kinds of issues that we were able to overcome via
reinforcement learning.


\insertRealResults

